Current and Future Use of Large Language Models for Knowledge Work

Large Language Models (LLMs) have introduced a paradigm shift in interaction with AI technology, enabling knowledge workers to complete tasks by specifying their desired outcome in natural language. LLMs have the potential to increase productivity and reduce tedious tasks in an unprecedented way. A systematic study of LLM adoption for work can provide insight into how LLMs can best support these workers. To explore knowledge workers' current and desired usage of LLMs, we ran a survey (n=216). Workers described tasks they already used LLMs for, like generating code or improving text, but imagined a future with LLMs integrated into their workflows and data. We ran a second survey (n=107) a year later that validated our initial findings and provides insight into up-to-date LLM use by knowledge workers. We discuss implications for adoption and design of generative AI technologies for knowledge work.

==> 0_abstract.tex <==
%150 words max
%stand current usage, perceptions of LLMs, and desired future usage in the context of knowledge work, we ran a survey (n=216) at a large technology company in Summer 2023. 
%Approximately a quarter of participants had used LLMs for work, while 55\% had used LLMs outside of work and 84\% would like to use LLMs for work in the future.
%Participants described discrete work tasks they had already used LLMs for, like generating a code template or improving a snippet of text, while they imagined a future where LLMs are integrated into their work and data, like assistance with handling their calendar and emails. Yet, workers' main concerns are with the output reliability and data privacy. 
%We discuss our findings in the context of the future of AI technologies for knowledge work.

Large Language Models (LLMs) have introduced a paradigm shift in interaction with AI technology, enabling knowledge workers to complete tasks by specifying their desired outcome in natural language. LLMs have the potential to increase productivity and reduce tedious tasks in an unprecedented way. A systematic study of LLM adoption for work can provide insight into how LLMs can best support these workers. To explore knowledge workers' current and desired usage of LLMs, we ran a survey (n=216). Workers described tasks they already used LLMs for, like generating code or improving text, but imagined a future with LLMs integrated into their workflows and data. We ran a second survey (n=107) a year later that validated our initial findings and provides insight into up-to-date LLM use by knowledge workers. We discuss implications for adoption and design of generative AI technologies for knowledge work.




%%%%% OLD VERSION-----------------------------------------
%%%%%%%
% The recent availability of ChatGPT and other text-to-text large language models (LLMs) has the potential to change the way people work. 
% Despite significant technological advances for workers in the past few decades, Large Language Models (LLMs) could further support productivity and reduce tedious tasks.
%there are still many opportunities for supporting knowledge workers.
%Recent advances in text-to-text large language models offer promise in many domains and likely can accelerate knowledge work practices.
% Workers are already beginning to use LLMs for their work, but a systematic study of adoption of LLMs for work can provide deeper insight into the needs of workers and future directions for LLM support of work.
% However, we know little about how people are currently using LLMs for their work, how they imagine using LLMs for their work in the future, and what is preventing people from using LLMs. 
% To better understand usage and perceptions of LLMs in the context of knowledge work, we ran a survey (n=216) at a large technology company in Summer 2023. 
% Approximately a quarter of participants had used LLMs for work, while 55\% had used LLMs outside of work and XX\% would like to use LLMs for work in the future.
% We found that participants currently describe discrete tasks in which they request templates or drafts from an LLM. 
% While users imagine a future where LLMs are integrated into their work and data, their main concerns are with the output reliability and data privacy. 
% We discuss our findings in the context of the future of AI technologies for knowledge work.
%What we're doing: understanding usage and perceptions of LLMs in the context of knowledge work






==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> tables/3_tab_demographics.tex <==




\begin{table}[h!]
    \caption{Participant demographics of all  Survey1 \color{black}participants (n=216). We list all job roles in the table with more than one participant listing them. Participants also listed several other roles, like content creation,  education, audit, communications, operations, strategy, content writing, contract preparation, procurement, and proposal management.}
    \begin{tabular}{c | c} % for the center line
    \hline
            \begin{tabular}[t]{lll}
                % \toprule
                % \multicolumn{2}{}{Work locations}\\ \hline
                Work Location (select one)& \# & \%\\ \hline
                North America &136&63\%\\ 
                Europe &47&22\%\\ 
                Asia &22&10\%\\ 
                South America &5&2\%\\ 
                Oceania &3&1\%\\ 
                Africa &3&1\%\\ 
      
                \hline
                AI experience (select all that apply)& \# & \%\\ \hline
                Tried consumer AI tools  &151&70\%\\ 
                Use consumer AI systems regularly &92&43\%\\ 
                Closely follow AI news &86&40\%\\ 
                Some work experience/education &69&32\%\\ 
                Work related to AI &53&25\%\\ 
                Significant AI work experience &26&12\%\\ 
                Don't know much about it &17&8\%\\ 
    
            \end{tabular}
        &
            \begin{tabular}[t]{lll}
            % \toprule
                Job Responsibility (select all that apply)& \# & \%\\ \hline
                Technical &97&45\%\\ 
                Design &41&19\%\\ 
                Sales &35&16\%\\ 
                Research & 28 & 13\% \\ 
                Analyst &27&12\%\\ 
                User Research &24&11\%\\ 
                Marketing &24&11\%\\ 
                Management &18&8\%\\
                Customer Service &15&7\%\\ 
                Product/project Management &12&6\%\\ 
                Administrative & 10 & 5\% \\ 
                Human Resources  &6&3\%\\ 
                Executive &4&2\%\\ 
                Finance & 3 & 1\% \\
                Copy editing & 3 & 1\% \\ 
                Consulting & 3 & 1\% \\ 
                Legal &2&1\%\\
                Accounting & 2 & 1\% \\ 
            \end{tabular}
            \\ \hline
    \end{tabular}
    \label{tab-demo}
\end{table}



\begin{table}[h!]

    \caption{Participant demographics of all participants for Survey2 (n=107). We list all job roles in the table with more than one participant listing them. Participants also listed several other roles, like Hardware Development \& Support, Legal, Site Reliability Engineer, Technical Services, Supply Chain, and Research. Note that due to policies, the work location and job responsibility questions required slight modifications from Survey1.}
    \begin{tabular}{c | c} % for the center line
    \hline
            \begin{tabular}[t]{lll}
                % \toprule
                % \multicolumn{2}{}{Work locations}\\ \hline
                Work Location (select one)& \# & \%\\ \hline
                Americas &56&52\%\\ 
                EMEA (Europe, the Middle East, and Africa) &42&39\%\\ 
                APAC (Asia Pacific)   &9&8\%\\ 
      
                \hline
                AI experience (select all that apply)& \# & \%\\ \hline
                Tried consumer AI tools  &71&66\%\\ 
                Use consumer AI systems regularly &44&41\%\\ 
                Closely follow AI news &34&32\%\\ 
                Some work experience/education &47&44\%\\ 
                Work related to AI &31&29\%\\ 
                Significant AI work experience &8&4\%\\ 
                Don't know much about it &9&8\%\\ 
    
            \end{tabular}
        &
            \begin{tabular}[t]{lll}
            % \toprule
                Job Responsibility (select all that apply)& \# & \%\\ \hline
                Software Development \& Support&   22& 21\%\\
                Consultant&                        13& 12\%\\
                Technical Sepcialist &             10& 9\%\\
                Finance   &                         8& 7\%\\
                Marketing \& Communications &       7& 7\%\\
                Enterprise Operations &             5&  5\%\\
                Sales           &                   5&  5\%\\
                Project Management  &               5&   5\%\\
                Architect        &                  5&  5\%\\
                Human Resources  &                   3& 3\%\\
                Design         &                     3& 3\% \\
                Information Technology \& Services&  3&  3\% \\
                Communications          &            3&  3\% \\
                Offering Management    &             3&  3\% \\
                Data Science          &              2&   3\% \\
                General Management    &              2&  3\% \\
            \end{tabular}
            \\ \hline
    \end{tabular}
    \label{tab:demo2}
\end{table}


==> tables/4_tab_demographic_stats.tex <==
% \begin{table}[]
%     \caption{Participant demographics of all participants (n=216)}
%     \begin{tabular}{c | c} % for the center line
%     \hline
%             \begin{tabular}[t]{lll}
%                 % \toprule
%                 % \multicolumn{2}{}{Work locations}\\ \hline
%                 Work Location (select one)& \# & \%\\ \hline
%                 North America &136&63\%\\ 
%                 Europe &47&22\%\\ 
%                 Asia &22&10\%\\ 
%                 South America &5&2\%\\ 
%                 Oceania &3&1\%\\ 
%                 Africa &3&1\%\\ 
      
%                 \hline
%                 AI experience (select all that apply)& \# & \%\\ \hline
%                 Tried consumer AI tools  &151&70\%\\ 
%                 Use consumer AI systems regularly &92&43\%\\ 
%                 Closely follow AI news &86&40\%\\ 
%                 Some work experience/education &69&32\%\\ 
%                 Work related to AI &53&25\%\\ 
%                 Significant AI work experience &26&12\%\\ 
%                 Don't know much about it &17&8\%\\ 
    
%             \end{tabular}
%         &
%             \begin{tabular}[t]{lll}
%             % \toprule
%                 Job Responsibility (select all that apply)& \# & \%\\ \hline
%                 Technical &97&45\%\\ 
%                 Design &42&19\%\\ 
%                 Management &29&13\%\\ 
%                 Analyst &27&12\%\\ 
%                 Sales &34&16\%\\ 
%                 User Research &24&11\%\\ 
%                 Marketing &24&11\%\\ 
%                 Customer Service &15&7\%\\ 
%                 Product Management &9&4\%\\ 
%                 Human Resources  &6&3\%\\ 
%                 Executive &4&2\%\\ 
%                 Legal &2&1\%\\
%                   & \\
%                 & \\
%             \end{tabular}
%             \\ \hline
%     \end{tabular}
%     \label{tab-demo}
% \end{table}


\begin{table}[h]
    \caption{AI experience statistics(n=216). To reduce complexity, we only show significant combinations of post-hoc comparisons. }
    \begin{tabular}{p{2cm} p{3.5cm} p{1cm} p{3.5cm} p{3.5cm} } % for the center line
    \hline
        
    AI experience (select all that apply)&Overall &  &  tried-it & no-use\\ \hline
    \multirow{2}{2cm}{Tried consumer AI tools}  & \multirow{2}{3.5cm}{$\chi^2 (3,212)=29.4, p<.001$} & personal& n.s. & $\chi^2 (1,103)=21.2, p<.008$\\ 
      && tried-it & - &  $\chi^2 (1,101)=16.6, p<.008$\\ \hline

      
     \multirow{3}{2cm}{Use consumer AI systems regularly}  & \multirow{2}{3.5cm}{$\chi^2 (3,212)=44.8, p<.001$}&   work &$\chi^2 (1,109)=27.1, p<.008$ & $\chi^2 (1, 96) =22.3, p<.008$ \\ 
     & & personal & $\chi^2 (1,116)=17.6, p<.008$ & $\chi^2 (1, 103)=14.0, p<.008$  \\ 
     & & \\ \hline

     Significant AI work exp. & $\chi^2 (3,212)=15.6, p<.01$& work &$\chi^2 (1, 109)=10.1, p<.008$ & n.s.\\ \hline

     \multirow{2}{2cm}{Don't know much about it}  & \multirow{2}{3.5cm}{$\chi^2 (3,212)=23.3, p<.001$}& work & n.s. &  $\chi^2 (1,96)=12.2, p<.008$\\ 
     && personal & n.s.& $\chi^2 (1,103)=8.7, p<.008$ \\ \hline
    Work related to AI  & $\chi^2 (3,212)=0.7, p=.87$& - & -& -\\ \hline
   Closely follow AI news & $\chi^2 (3,212)=5.5, p=.14$& - & -& -\\ \hline
   Some work exp./ education& $\chi^2 (3,212)=6.3, p=.1$& - & -& -\\ \hline
       

    \end{tabular}
    \label{tab:demo-stats}
\end{table}

==> tables/4_tab_domains.tex <==


\begin{table}[]
\caption{Percentage of each group who described tasks in each of the four domains for tasks they currently use LLMs for and work tasks they would like to use LLMs for in an ideal future}~\label{tab:domain}
\small
\begin{tabular}{p{5cm}|lll|llll}
\toprule
& &Current & &  &Future & \\
Domain & Work  & Personal& Tried-it & Work & Personal & Tried-it & No-use \\ \hline
\textbf{Technical}: related to code or IT &45\% & 13\% & 19\% &47\% & 20\% & 24\% & 29\%\\
\textbf{General}: no domain specified & 17\% &35\% &40\% &32\% &32\% & 31\% & 33\% \\
\textbf{Specialized} (non-technical): e.g. as sales, HR &34\% &75\% & 48\%  & 15\% &25\% & 22\% & 7\% \\
\textbf{Communication}: e.g. email, messages & 9\% & 10\% & 3\% & 25\% & 20\% & 10\%& 11\% \\
\bottomrule
\end{tabular}
\end{table}


% \begin{table}[]
% \caption{Percentage of each group who described tasks in each of the four domains for tasks they currently use LLMs for and work tasks they would like to use LLMs for in an ideal future}~\label{tab:domain}
% \small
% \begin{tabular}{l|l ll|lll}
% \toprule
% & &Current & &  &Future & \\
% Domain & Work-use  & Personal-use & Tried-it & Work-use  & Personal-use & Tried-it \\ \hline
% Technical & 45\% & 13\% & 19\% & +2\% & +7\% & \cellcolor{light-gray}+5\% \\
% General & 17\% &\cellcolor{light-gray} 35\% &\cellcolor{light-gray}  40\% &\cellcolor{light-gray} +15\% &\cellcolor{med-gray} -3\% & \cellcolor{med-gray}+9\% \\
% Specialized non-technical &\cellcolor{light-gray} 34\% &\cellcolor{med-gray} 75\% & \cellcolor{med-gray} 48\%  & -19\% &\cellcolor{light-gray} -50\% & -26\%\\
% Communication & 9\% & 10\% & 3\% & +14\% & +10\% & +7\%\\
% \bottomrule
% \end{tabular}
% \end{table}

==> tables/4_tab_frustrations_concerns.tex <==
\begin{table}[h]
\caption{Frustrations with current work and personal use and concerns for future use of LLMs at work. We provide percentages of each adoption group that mentioned the frustrations and concerns. Since some participants mentioned multiple, columns may add to more than 100\%.}~\label{tab:frustrations_concerns}
\small
\begin{tabular}{p{1cm}|p{6.5cm}|p{.75cm}p{1cm}|p{.75cm}p{.75cm}p{.75cm}p{.75cm} }
\toprule
& & Current &Frustrations  & & Future& Concerns& \\
Theme & Frustration/Concern & Work-use & Personal & Work-use & Personal & Tried-it & No-use \\ \hline
Output & Unreliable: the outputs are incorrect or not reliably correct & 43\% & 45\% & 32\% & 30\% & 33\%  & 42\%   \\

& Style: the way the output is written is inappropriate or could be improved& 8\% & 22\% & 2\% & 5\% & 3\%  & 4\%  \\

&Black box: there is no information about how the system arrived at the output & 4\% & 2\% & 6\% & 3\% & 7\%  & 11\%  \\ \hline
Data & Privacy: concern about who has access to data that is exposed to an LLM&  8\% & 7\% & 42\% & 43\% & 40\%  & 24\%   \\
& Policies: discussion of company rules that impact LLM usage & 13\% & 0\% & 6\% & 12\% & 10\%  & 7\%  \\
& Specialized knowledge: the LLM does not have particular or up-to-date knowledge about a topic& 9\% & 15\% & 2\% & 7\% & 0\%  & 4\%    \\
& Training data: concerns about the data the LLM has been trained on, such as problematic biases on the internet or just factually incorrect data& 4\% & 0\% & 4\% & 7\% & 10\%  & 24\%  \\
 \hline
Usability & Prompting: difficulties determining how to specify the task&23\% & 13\% & 2\% & 0\% & 3\%  & 0\%   \\ 
&Review effort: a high amount of effort is needed to check over the output of the LLM& 2\% & 3\% & 6\% & 2\% & 5\%  & 7\%  \\
& Setup: setting up or understanding how to set up the LLM is challenging or not straightforward&  2\% & 5\% & 4\% & 7\% & 5\%  & 2\%   \\
& Other: other usability, like the LLM refusing to answer&  15\% & 12\% & 4\% & 2\% & 0\%  & 2\% \\ \hline
Individual  
& Ownership: concerns about whether the user will have rights to the LLM output &  2\% & 3\% & 9\% & 7\% & 16\%  & 7\%  \\
& Job: concerns about a role not being needed at all or as much due to LLMs&0\% & 2\% & 6\% & 3\% & 12\%  & 4\%   \\
& Skills: not wanting to lose skills by offloading work to a system&0\% & 0\% & 6\% & 5\% & 9\%  & 13\%  \\
& Enjoy: workers enjoy writing and do not want to offload it& 0\% & 0\% & 0\% & 0\% & 2\%  & 9\%   \\
 \hline
Societal& Ownership: LLMs have potentially been trained on copyrighted data without acknowledging the owners or providing payment&0\% & 2\% & 4\% & 3\% & 5\%  & 4\%  \\
& Bias: LLMs can potentially reinforce biases at a societal level due to their far reach&  0\% & 0\% & 0\% & 2\% & 3\%  & 0\%  \\
& Other: such as environmental& 0\% & 2\% & 6\% & 3\%& 2\%  & 4\%  \\
\bottomrule
\end{tabular}
\end{table}


==> tables/4_tab_task_type_counts.tex <==


\begin{table}[]
\caption{\color{magenta}Theme counts: Current}~\label{tab:task-counts}
\small
\color{magenta}
\begin{tabular}{p{1.25cm}p{1.25cm} p{1cm} p{1cm} p{1cm} | p{1cm} p{1cm} p{1cm} | p{1cm} p{1cm} }
\toprule

Theme & Sub-Theme  & Current Study1- work & Current Study1- personal& Current Study1- tried-it & Current Study2- work & Current Study2- personal& Current Study2- tried-it & Future Study1 (work)& Future Study2 (work)\\
\hline
\multirow{2}{*}{Creation} & Artifact   \\
& Idea &  \\ \hline
\multirow{2}{*}{Information} & Search   \\
& Learn &  \\
& Summarize &  \\
& Analyze &  \\ \hline
\multirow{3}{*}{Advice} & \\
& Guidance & \\
& Validation &  \\ \hline

Automation& Automation &  \\


\bottomrule
\end{tabular}
\end{table}




==> tables/4_tab_task_types.tex <==


\begin{table}[]
\caption{Themes and sub-themes for LLM usage }~\label{tab:task-types}
\small
\begin{tabular}{llp{8cm}l}
\toprule
Theme & Sub-Theme & Description & Current, Future, or Both \\
\hline
\multirow{2}{*}{Creation} & Artifact & Generate a new artifact to be used directly or with some modification (such as an email, code, a blog post, marketing content) & Both \\
& Idea & Generate an idea, to be used indirectly & Both \\ \hline
\multirow{2}{*}{Information} & Search & Seek a fact or piece of information & Both \\
& Learn & Learn about a new topic more broadly (like Kubernetes)& Both \\
& Summarize & Generate a shorter version of a piece of content that describes the important elements. & Both \\
& Analyze & Discover new information about a set of information or data. & Both \\ \hline
\multirow{3}{*}{Advice} & Improve & Generate a better version (like improved grammar or improved code) & Both \\
& Guidance & Get guidance about how to make a decision.& Both \\
& Validation & Check whether an artifact satisfies a set of rules or constraints. & Both \\ \hline

Automation& Automation & Complete a task in a piece of software with less or no human effort. & Future \\


\bottomrule
\end{tabular}
\end{table}


==> tables/4_tab_tasks.tex <==
\begin{table}[h]
\caption{Types of support workers want from LLMs for current LLM usages and usages of LLMs in an ideal future. We report the percentage of each adoption group that discussed each task type. Some Participants described multiple tasks, leading to column percentages adding up to over 100\%.}~\label{tab:tasks}
\small
\begin{tabular}{p{1.5cm}|p{4.5cm}|p{.75cm}p{1cm}p{.75cm}|p{.75cm}p{.75cm}p{.75cm}p{.75cm}}
\toprule
& & &Current  & & &Future & \\
Theme & LLM Assistance Type & Work-use & Personal-use & Tried-it& Work-use & Personal-use & Tried-it  & No-use\\ \hline
\multirow{2}{1cm}{Creation} & \textbf{Artifact}: Generate text. & 51\% & 42\% &47\%  & 66\% & 50\% & 50\%   & 40\%   \\
& \textbf{Idea}: Generate inspiration or brainstorm ideas. & 15\% & 27\% & 10\%  & 19\% & 8\% & 10\% & 2\%  \\ \hline
% & \textbf{Other}: Generate a non-text element & 0 & 0 & 5\% \\ \hline
\multirow{2}{1cm}{Informa-tion} & \textbf{Search}: Retrieve or collect information. & 23\% & 17\% & 38\%  & 15\% & 13\% & 12\% & 20\%  \\
 & \textbf{Learn}: Get an explanation of a concept. &11\% & 15\% & 7\%  & 8\% & 2\% & 3\%  & 2\%    \\ \hline

\multirow{3}{1cm}{Advice} & \textbf{Improve}: Get an improved version of an artifact &  23\% & 20\% & 0\%  & 13\% & 13\% & 3\% & 4\%   \\
 & \textbf{Guidance}: Get a recommendation   &  6\% & 13\% & 2\%  & 9\% & 3\% & 3\%  & 13\%   \\
 & \textbf{Validation}: Check that a set of criteria is met  &  2\% & 2\% & 0\%  & 9\% & 0\% & 2\%   & 16\%    \\ \hline

\multirow{2}{1cm}{Sense-making} & \textbf{Summarize}: Get the main idea.  & 17\% & 12\% & 2\%  & 15\% & 23\% & 7\%  & 4\%   \\
 & \textbf{Analysis}: Get new insights about information.  &  6\% & 2\% & 0\%  & 13\% & 10\% & 12\%   & 4\%    \\ \hline
 Automation & \textbf{Automation}: Perform actions for a user.  &  0\% & 0\% & 0\%  & 17\% & 17\% & 12\%  & 13\%      \\

\bottomrule
\end{tabular}
\end{table}


==> tables/4_tab_use_of_LLMs.tex <==
% \begin{table}[]
% \caption{Responses to how participants have used LLMs, including responses from the full set of 335 participants who responded to this question}~\label{tab:use}
% \small
% \begin{tabular}{l|l|l}
% \toprule
% Response & Count & Percentage  \\ \hline
% \textbf{All who have used for work} &\textbf{53} &\textbf{24.5\%} \\
% \hspace{3mm}For work and non-work and trying it out &\hspace{1mm}25& \\
% \hspace{3mm}For work and non-work &\hspace{1mm}20 & \\
% \hspace{3mm}For work and trying it out &\hspace{1mm}4& \\ 
% \hspace{3mm}For work &\hspace{1mm}4 & \\ \hline
% \textbf{All who have used for non-work} &\textbf{60} &\textbf{27.8\%}  \\
% \hspace{3mm}For non-work and trying it out &\hspace{1mm}41 & \\ 
% \hspace{3mm}For non-work &\hspace{1mm}19 & \\ \hline
% \textbf{Just trying it out}&\textbf{58} & \textbf{26.9\%} \\
% \textbf{Have not used} &\textbf{45} &\textbf{20.8\%} \\ \hline
% Total&216& 100\% \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[tb]
\caption{Adoption groups, along with average programming experience and percentage of each group with significant AI work experience for Survey1 (S1, n=216) and Survey2 (S2, n=107)\color{black}. }~\label{tab:use}
\small
\begin{tabular}{p{.5cm}p{.75cm}p{.5cm}p{.75cm}p{1.5cm}p{2.5cm}p{1.5cm}|p{2cm}p{1.5cm}}
\toprule
Used for work & Used outside of work & Tried it & Haven't used & Count  (S1 total: 216, S2 total: 107) \color{black}& Percentage &Group Name & Programming Exp. (1-10) & \% Significant AI work experience \\ \hline
\checkmark & \checkmark & \checkmark & - 
        & S1:\color{black}25 S2:10 &  \multirow{4}{2.5cm}{S1:\color{black}24.5\%  S2: 34.6\%\color{black}} 
        & \multirow{4}{*}{\textit{work-use}} & \multirow{4}{2cm}{ S1:\color{black}M=6.1,SD =3.2 S2:M=4.3,SD=2.8}& \multirow{4}{1.5cm}{ S1:\color{black}26\% S2:14\%}\\
\checkmark & \checkmark & - & -&  S1:\color{black}20 S2:19& & \\
\checkmark &-  & \checkmark & -& S1:\color{black}4 S2:4& & \\ 
\checkmark &-  & - &- & S1:\color{black}4 S2:4& & \\\hline

-& \checkmark & \checkmark & -
        & S1:\color{black}41 S2:10 & \multirow{2}{2.5cm}{S1:\color{black}27.8\% S2:29.9\%} 
        & \color{black}\multirow{2}{*}{\textit{personal-use}} & \multirow{2}{2cm}{S1:\color{black}M=4.6,SD=3.3 S2:M=4.8,SD=3.1}& \multirow{2}{1.5cm}{S1:\color{black}12\% \hspace{1mm}S2:9\%}\\
-& \checkmark &- & -&   S1:\color{black}19 S2:22 & & \\\hline

- & - & \checkmark &-
        & S1:\color{black}58 S2:29 & S1:\color{black}26.9\% S2:27.1\%
        & \color{black} \textit{tried-it} &  S1:\color{black}M=5.2,SD=3 S2: M=5.6,SD=3.7 &  S1:\color{black}3\% \hspace{2mm}S2:0\%  \color{black}\\ \hline

\color{black}-& - & - & \checkmark 
        &  S1:\color{black}45 S2:9 &  S1:\color{black}20.8\% S2:8.4\% 
        & \color{black}\textit{no-use} &  S1:\color{black}M=4.5,SD=3.2 S2:M=5.2,SD=3.9& S1:\color{black}7\% \hspace{2mm}S2:0\%\color{black}\\
\bottomrule
\color{black}
\end{tabular}
\color{black}
\end{table}

% \textbf{All who have used for work} &\textbf{37} &\textbf{34.6\%} \\
% \hspace{3mm}For work and non-work and trying it out &\hspace{1mm}10& \\
% \hspace{3mm}For work and non-work &\hspace{1mm}19 & \\
% \hspace{3mm}For work and trying it out &\hspace{1mm}4& \\ 
% \hspace{3mm}For work &\hspace{1mm}4 & \\ \hline
% \textbf{All who have used for non-work} &\textbf{32} &\textbf{29.9\%}  \\
% \hspace{3mm}For non-work and trying it out &\hspace{1mm}10 & \\ 
% \hspace{3mm}For non-work &\hspace{1mm}22 & \\ \hline
% \textbf{Just trying it out}&\textbf{29} & \textbf{27.1\%} \\
% \textbf{Have not used} &\textbf{9} &\textbf{8.4\%} \\ \hline
% Total&107& 100\%\\


% For work & & \\
% For work and non-work & & \\
% For work and non-work and trying it out & & \\
% For work and trying it out & & \\
% All who have used for work  & & \\
% For non-work & & \\
% For non-work and trying it out & & \\
% All who have used for non-work & & \\
% Just trying it out & & \\
% Have not used & & \\

==> tables/4_tab_why_not_use.tex <==
\begin{table}[tb]
\caption{Multiple choice responses to why participants had not used LLMs or why they had not used LLMs for a work or non-work task (only no-use and tried-it participants answered this question). }~\label{tab:nouse}
\small
\begin{tabular}{l|p{3.5cm}|p{3.5cm}}
\toprule
Response & No-use & Tried-it \\ \hline
I have privacy concerns& 46\% & 63\%\\
I have concerns with the ownership of the output of the LLM. & 46\% & 54\%\\
I don’t trust it& 42\% & 51\%\\
I can’t think of a task to use it for & 36\% & 28\%\\
I’m waiting for the technology to improve. & 30\% & 39\% \\
I don’t have time & 25\% & 21\% \\
I don’t want to pay for it & 11\% & 15\% \\
I don’t know what an LLM/ChatGPT is. & 2\% & 0\% \\
\bottomrule
\end{tabular}
\end{table}


==> tables/discussion-table.tex <==
\begin{table}[b]
\caption{Support and expansion of prior work with our findings }~\label{tab:discussion}
\small
\begin{tabular}{lll}
\toprule
Theme & Sub-Theme & Prior work that includes this type of LLM task \\
\hline
\multirow{2}{*}{Creation} & Artifact & work~\cite{ritala2023transforming}, writing~\cite{gmeiner2023dimensions}, education~\cite{yan2023practical},  general~\cite{skjuve2023user, taecharungroj2023can, skjuve4376834people}\\
& Idea &  work~\cite{ritala2023transforming}, programming~\cite{ross2023programmer}, general~\cite{skjuve2023user,taecharungroj2023can,skjuve4376834people}\\ \hline
\multirow{2}{*}{Information} & Search & work~\cite{ritala2023transforming}, programming~\cite{ross2023programmer}, general~\cite{skjuve2023user,taecharungroj2023can,skjuve4376834people}\\
& Learn & work~\cite{ritala2023transforming}, programming~\cite{ross2023programmer}, general~\cite{skjuve2023user,taecharungroj2023can,skjuve4376834people}\\
& Summarize &   writing~\cite{gmeiner2023dimensions} \\
& Analyze & education~\cite{yan2023practical}, healthcare~\cite{zheng2023innovating}\\ \hline
\multirow{3}{*}{Advice} & Improve & work~\cite{ritala2023transforming}, programming~\cite{ross2023programmer}, writing~\cite{gmeiner2023dimensions}\\
& Guidance &  education~\cite{yan2023practical}, healthcare~\cite{zheng2023innovating}\\
& Validation & education~\cite{yan2023practical} \\ \hline

Automation& Automation & work~\cite{ritala2023transforming} \\


\bottomrule
\end{tabular}
\end{table}

% Researchers have combinations of our LLM uses in current general use of LLMs~\cite{skjuve2023user, taecharungroj2023can, skjuve4376834people}, as well as particular contexts like writing~\cite{gmeiner2023dimensions}, programming~\cite{ross2023programmer}, healthcare~\cite{zheng2023innovating}, and education~\cite{yan2023practical}.

% Outside of work, researchers have found common LLM usages via twitter include writing of a variety of types (creation-artifact) and answering questions (information-search) ~\cite{taecharungroj2023can} and via a study include creative work (creation-artifact, creation-ideas), learning (information-learn), for writing and code generation (creation-artifact), as well as for fun, novelty and social support. 

% In the writing space, researchers outlined a set of LLM capabilities that would be valuable: which have some overlap with our results: text summarization (information-summarize), paraphrasing/rewriting (advice-improve), dialog generation (creation-artifact), sentence completion and elaboration (creation-artifact), formatting (information-summarize), story seeding and keyword association (creation-idea) ~\cite{gmeiner2023dimensions}. 

% In the code space, researchers also found that participants wanted to use a conversational assistant backed by an LLM for lookup (information-search), generating and explaining code (creation-artifact), and supporting them in understanding what code does (information-learn) ~\cite{ross2023programmer}. This study also found some forward-thinking about the value of LLMs in code, suggesting that features like refactoring would be helpful, similar to some of our results about future uses of LLMs. 

% The closest work to ours, which covered interviews of knowledge workers outlined a set of knowledge work tasks that LLMs can support that align with 6 of the 10 types of LLM usage that we describe: answering questions (aligns with our information-search), providing inspiration (creation-idea), content production (creation-artifact), content reorganization (advice-improve), write and improve code (creation-artifact, advice-improve), learning (information-learn), generate emails and communications (creation-artifact), repetitive tasks (automation) ~\cite{ritala2023transforming}.

% While ~\cite{skjuve2023user} did not focus on systematically categorizing usage in the way that we did, they list several ways their users talked about using ChatGPT: answering questions (information-search), generating content (creation-artifact), learning (information-learn), participating in creative work such as idea generation (creation-idea). 




%\cite{skjuve4376834people} : search, artifact generation, idea, learn, 


==> tables/type_of_use.tex <==
\begin{table}[]
\caption{}~\label{tab:typeOfUse}
\small
\begin{tabular}{l|l|l|l}
\toprule
LLM Output Type & Work & Nonwork & Tryit  \\ \hline
\textbf{Generation} text & &\textbf\\
\hspace{3mm} ideas && \\
\hspace{3mm} other & & \\
\textbf{Generation} text & &\textbf\\
\hspace{3mm} ideas && \\
\hspace{3mm} other & & \\
\bottomrule
\end{tabular}
\end{table}

